Model-Agnostic Meta-Learning for Multilingual Hate Speech Detection

Hate speech in social media is a growing phenomenon, and detecting such toxic content has recently gained significant traction in the research community. Existing studies have explored fine-tuning language models (LMs) to perform hate speech detection, and these solutions have yielded significant performance. However, most of these studies are limited to detecting hate speech only in English, neglecting the bulk of hateful content that is generated in other languages, particularly in low-resource languages. Developing a classifier that captures hate speech and nuances in a low-resource language with limited data is extremely challenging. To fill the research gap, we propose HateMAML, a model-agnostic meta-learning-based framework that effectively performs hate speech detection in low-resource languages. HateMAML utilizes a self-supervision strategy to overcome the limitation of data scarcity and produces better LM initialization for fast adaptation to an unseen target language (i.e., cross-lingual transfer) or other hate speech datasets (i.e., domain generalization). Extensive experiments are conducted on five datasets across eight different low-resource languages. The results show that HateMAML outperforms the state-of-the-art baselines by more than 3% in the cross-domain multilingual transfer setting. We also conduct ablation studies to analyze the characteristics of HateMAML.

==> Discussion.tex <==
\textcolor{red}{ Discussion on baselines, strength and weeknesses. zeroshot vs fewshot.} 
% \textcolor{red}{Eshaan}: Rough notes on X-MAML results. Some primary thoughts on model performance.
% \begin{itemize}
%   \item Zero-Shot (SemEval 2020)
%   \begin{itemize}
%       \item X-MAML is able to improve upon the results in Arabic and Turkish (mag of 0.015 and 0.017)
%       \item For Greek the improvement is minuscule. Can be attributed to:-
%       \begin{itemize}
%           \item X-MAML being too reliant on auxiliary language compatibility. As this is not the case for HateMAMAL (i.e it is able to improve its performance better), does this mean it is more general?
%       \end{itemize}
%       \item For Danish results show no change.
%       \item Greek seems to be the best auxiliary language, But no language was able to compliment Greek the best... impelling the concept of auxiliary language not only depend on language family, but also the quality of dataset.
%   \end{itemize}
  
%   \item Few-Shot (SemEval 2020)
%   \begin{itemize}
%       \item If we consider MAML as a "model initialisation" task X-MAMAL is able to do it best(AS OF NOW), but in all these results danish was the auxiliary language 
%   \end{itemize}
% \end{itemize}
% \textcolor{red}{Rabiul}: Compare proposed model performance with baselines.


% \textcolor{purple}{Start wrapping up discussions from rough notes written by all of us. Put them into proper context. Can start ftom Oct 27. [Tanmay]}


==> Preliminaries.tex <==
\subsection{Problem statement}
In this paper, we deal with the binary classification task of hate speech detection.
%Each train or evaluation example consists of the text content of the comment and its hate label.
In the zero-shot scenario, given a source language training set,
the task is to learn a classification model that performs well on a previously unseen target evaluation set.
Moreover, multiple additional auxiliary language datasets can also be utilized.
In the few-shot setting, we can additionally utilize a small target dataset to help incorporate language specific knowledge to the model's training procedure.
Finally, in our experiments, we also explore a self-training algorithm. Instead of requiring an additional small labeled dataset as defined above, for self-training we simply require an unlabeled set of comments.

% \subsection{Source, auxiliary and target language}
% \textbf{Source language} - The language that acts as a source in cross-lingual transfer to a target low-resource language. Generally, the source language should be high-resourced, such as English.
% \textbf{Auxiliary language} - An auxiliary language that assists meta-learning hate tasks for the target language (similar to \cite{nooralahzadeh-etal-2020-zero, gu-etal-2018-meta}). 
% \textbf{Target language} - Fine-tuned (or meta-tuned) model will be evaluated on the test set in the target low-resource language. We are mainly interested in model performance on chosen target languages. 
